Benchmarking and Analyzing 3D Human Pose and Shape Estimation Beyond Algorithms

3D human pose and shape estimation (a.k.a. "human mesh recovery") has achieved substantial progress. Researchers mainly focus on the development of novel algorithms, while less attention has been paid to other critical factors involved. This could lead to less optimal baselines, hindering the fair and faithful evaluations of newly designed methodologies. To address this problem, this work presents the first comprehensive benchmarking study from three under-explored perspectives beyond algorithms. 1) Datasets. An analysis on 31 datasets reveals the distinct impacts of data samples: datasets featuring critical attributes (i.e. diverse poses, shapes, camera characteristics, backbone features) are more effective. Strategical selection and combination of high-quality datasets can yield a significant boost to the model performance. 2) Backbones. Experiments with 10 backbones, ranging from CNNs to transformers, show the knowledge learnt from a proximity task is readily transferable to human mesh recovery. 3) Training strategies. Proper augmentation techniques and loss designs are crucial. With the above findings, we achieve a PA-MPJPE of 47.3 mm on the 3DPW test set with a relatively simple model. More importantly, we provide strong baselines for fair comparisons of algorithms, and recommendations for building effective training configurations in the future. Codebase is available at http://github.com/smplbody/hmr-benchmarks

==> Figs/aug-results.tex <==
\begin{figure}[h!]

    \centering
    \subfigure{
    \includegraphics[width=0.45\linewidth,height=2in]{Figures/Aug/h36m-benchmarks.png}
    }
    \subfigure{
    \includegraphics[width=0.45\linewidth,height=2in]{Figures/Aug/coco-benchmarks.png}
    }
    \caption{Performance on various benchmarks when training with augmentation on (left) H36M and (right) EFT-COCO}
    \label{aug-perf}
\end{figure}


==> Figs/l1-results.tex <==
\begin{figure}[t]
    \vspace{-10pt}
    \centering
    \subfigure{
    \includegraphics[width=0.4\linewidth,height=1.6in]{Figures/Noise/l1-noise001.png}
    }
    \subfigure{
    \includegraphics[width=0.4\linewidth,height=1.6in]{Figures/Noise/l1-noise002.png}
    }
    \vspace{-5pt}    
\caption{\small \textbf{HMR model performance with and without L1 loss under different (a) proportions of noisy SMPL and keypoints; (b) ratios of noisy pose parameters.} }
\vspace{-15pt}
\label{l1-noise}
\end{figure}


==> Sections/0304_combine_backbones.tex <==

\section{Benchmarking Backbone Models}
\label{training-backbones}

\textbf{Model architecture.}
Following \citet{Kanazawa2017}, ResNet-50 \citep{He2016} is the default backbone in many mesh recovery works \citep{Joo2021, Kocabas2021, Kocabas2020, Kolotouros2019}. More recently, \citet{Kocabas2021} adopted HRNet-W32 \citep{Sun2019} and attributed the performance gains to its ability to produce  more robust high-resolution representations. We further consider other architectures. Particularly, we compare different variations of CNN-based models (ResNet-101, ResNet-152, HRNet, EfficientNet \citep{Tan2019}, ResNext \citep{Xie2016}), as well as the latest transformer-based architectures (ViT \citep{Dosovitskiy2021}, Swin \citep{Liu2021}, Twins (-SVT and -PCVCT) \citep{Chu2021}).
% It is a common practice to train the HMR model from a pre-trained backbone model. The quality of the adopted backbone model can significantly affect the performance of the resulting HMR model. 

\input{Tables/backbone}
Table \ref{table:backbone} reports the performance of the HMR model trained with different backbone architectures. First, increasing the backbone capacity allows deeper feature representations to be learned, yielding performance gains. For instance, the PA-MPJPE is reduced when we switch the backbone model from ResNet-50 to ResNet-152. This is consistent with the findings in \cite{Cai2021}. Second, transformer-based backbones are superior to CNN-based backbones, achieving lower PA-MPJPEs and similar FLOPs under comparable parameters (Table \ref{table:backbone}). They are capable of mining rich structured patterns, which are especially essential for learning from different data sources. This contradicts the discoveries in \cite{Cai2021}, which did not find the advantage of vision transformers over CNN-based ones.


\textbf{Weight initialization.}
It is common and computationally efficient to build the HMR model based on a pre-trained backbone. Initialization of the backbone model weights has a significant impact on the HMR model performance. PARE \citep{Kocabas2021} initializes the weights of the HRNet-W32 backbone from a pose estimation model trained on MPII. The initialized model is further finetuned on EFT-COCO for 175K steps before training on \emph{Mix 6}. \citet{Kocabas2021} noted that this strategy accelerates the model convergence and reduces overall training time. However, this study does not provide ablation studies to explore the effect of using pretrained weights from a pose estimation model.

\input{Tables/backbone-init}

To disclose the impact of weight initialization, we systematically benchmark strategies where the backbone weights are pre-trained with ImageNet, or from pose estimation models trained over MPII or COCO. The results are reported in Table \ref{backbone-init}. First, we observe that transferring knowledge from a strong pose estimation model is sufficient to achieve large improvement gains, and it is not necessary to further finetune the backbone with EFT-COCO. In Table \ref{backbone-init}, with the HRNet-W32 backbone and weights initialized from MPII, we can already achieve a PA-MPJPE of 51.5 \(mm\), which is very close to the error of 50.9 \(mm\) reported by PARE \citep{Kocabas2021}.
%This is without any part-guided attention mechanism and supervision from body part segmentation masks \citep{Kocabas2021}. 
The effectiveness of such a pretrained backbone suggests that features learnt from pose estimation tasks are robust and complementary for mesh recovery tasks. Second, the choice of the pose estimation dataset for weight initialization is also vital. Regardless of the backbone variants, pretraining the backbone with COCO gives better performance than MPII for different training dataset mixes and backbone architectures.

%\citet{Jiang2020} found that fine-tuning a model pre-trained on clean datasets aid in dealing with noisy labels. The better the pre-trained model is, the better it may generalize on downstream noisy training tasks. This could explain why useful pretrained weights assist the model in generalising to potentially noise features in a multi-dataset training.
\vspace{-5pt}
\begin{tcolorbox}[left=1mm, right=1mm, top=0.5mm, bottom=0.5mm, arc=1mm]
\textbf{Remark \#4:} The backbone architecture and weight initialization are vital for the HMR performance. Optimal configurations comprise of transformer-based backbones with weights initialized from a strong pose estimation model trained on in-the-wild datasets.
\end{tcolorbox}
\vspace{-5pt}

% The optimal configuration is the Twins backbone with weights initialized from a pose estimation model trained on the COCO datase

==> Sections/0304_combine_datasets.tex <==

\section{Preliminaries}

\textbf{Base model.} The origin of many mesh recovery works \citep{Kolotouros2019, Dwivedi2022, Kolotouros2021, Kocabas2020, Kocabas2021, Rajasegaran2021, Pavlakos, Luo2021} can be traced back to HMR \cite{Kanazawa2017}. It adopts a neural network to regress the parameters of a SMPL body \citep{Kanazawa2017}, which is a differentiable function that maps pose parameters $\theta$ and shape parameters $\beta$ to a triangulated mesh with 6980 vertices. Following this study, subsequent works have been built upon HMR to further enhance the recovery performance. For instance, some solutions are proposed to improve the robustness by adding an optimization loop \citep{Kolotouros2019}, estimating camera parameters \citep{Kocabas2022} or using probabilistic estimation to derive the pose \citep{Kolotouros2021}; some works also extend HMR to predict the appearance (e.g., HMAR \citep{Rajasegaran2021b}) or temporal dimension (e.g., HMMR \citep{Pavlakos2020}, VIBE \citep{Kocabas2020}, MEVA \citep{Luo2021}). We benchmark HMR as it has also been widely used as the baseline in many studies \cite{Patel2021, Joo2021, Cai2021, Dwivedi2022}. 

% The conclusions from our evaluations are general to other methods extended from HMR as well.
% %
% \lei{Will this claim, "xxx are general to methods extended from HMR", be too strong? As there seems not to be enough experiments to support it.}

\textbf{Evaluation.}
We follow the widely adopted evaluation protocol in \cite{Kanazawa2017,Kolotouros2019}. Performance is measured in terms of recovery errors (PA-MPJPE) in \(mm\).
%, which is the mean per joint position error after rigid alignment of the prediction with ground truth via Procrustes Analysis. 
A smaller PA-MPJPE value indicates better recovery performance.
%
We adopt the 3DPW \citep{Varol2017} test set for evaluation without any fine-tuning on its training set (\textit{Protocol 2})\footnote{Some works \citep{Kocabas2022, Zanfir2020, Luo2021, Lin2021, Sengupta2021, Gun-Hee2021} also adopt the 3DPW training set during training (\emph{Protocol 1}). In general, using the 3DPW training data improves the performance but it is not a universal practice.}. 
%Two public datasets are selected for evaluation. (1) 3DPW \citep{Varol2017} is a challenging outdoor dataset. 
%For real-world applications, it is preferable to create robust systems that can work under a wide variety of in-the-wild conditions. As such, 3DPW \citep{Varol2017} 
This outdoor dataset is often used as the main or only benchmark \citep{Kanazawa2017, Kolotouros2019, Sun2022, Dwivedi2022, Joo2021, Kocabas2020, Kocabas2021} to assess real-world systems under a wide variety of in-the-wild conditions.
We also evaluate the indoor H36M test set \citep{Ionescu2014}. The results can be found in the appendix, which gives the same conclusions as 3DPW. 
%is an indoor dataset and a common benchmark for 3D pose estimation tasks. 
%We adopt the training protocol in \cite{Kanazawa2017,Kolotouros2019} for all our benchmarks. 
%We evaluate on all videos of subjects 9 and 11 from all cameras. For each dataset, 
We train the model for 100 epochs\footnote{All models were trained with 8 Tesla V100 GPUs.} and evaluate its performance in each epoch. After this, the best PA-MPJPE is reported. 
%
We perform our benchmarking from three perspectives - datasets (Section \ref{training-datasets}), backbones (Section \ref{training-backbones}) and training strategies (Section \ref{training-strategies}).

\section{Benchmarking Training Datasets}
\label{training-datasets}
Training datasets play an important role in determining mesh recovery accuracy. 
% used in various human mesh recovery algorithms. Many works train on their own unique combination of datasets determined heuristically. They compare their model performance with other methods trained with different dataset mixes \citep{Kocabas2021, Kocabas2022, Joo2021, Li2021, Dwivedi2022}. Therefore, it is difficult to attribute the model performance to the proposed algorithm or to the handpicked selection of datasets. This necessitates benchmarks on different dataset selections.
%Prior works select datasets to train models in an empirical way. 
Table \ref{Dataset-mixes} in the appendix summarises the datasets used in various algorithms. Many works train on their own unique combinations of datasets determined heuristically \citep{Kocabas2021, Kocabas2022, Joo2021, Li2021, Dwivedi2022}. This makes it hard to attribute performance gains to the proposed algorithm or to the handpicked selection of datasets, and necessitates benchmarks on different dataset choices. We provide a systematic and comprehensive evaluation of the impact of training datasets on the HMR performance. Our benchmarks involve not only the datasets used in prior mesh recovery works, but also the newest ones (e.g., PROX \citep{Hassan2019}, AGORA \citep{Patel2021}) as well as those commonly used in 2D/3D pose estimation (e.g., LIP \citep{Gong2017}, Crowdpose \citep{Li2019}, AI Challenger \citep{Wu2017}, Penn-Action \citep{Zhang2013}, MuCo-3DHP \citep{Mehta2018}, etc.). 
%We consider two types of configurations: (1) using one single dataset to train the model; (2) combining multiple datasets to jointly train the model, which is commonly adopted in prior works. 
We consider different factors in the training datasets that can affect the model performance, which are rarely investigated previously. 

%(1) \textbf{Dataset attributes}. We identify the critical and non-critical attributes of the dataset in determining the mesh recovery accuracy. (2) \textbf{Dataset combinations}. Mixes of different datasets with different partitions can bring distinct performance gains, which encourages us to carefully select the optimal combination. (3) \textbf{Annotation quality}. In the real-world scenario, the collected data samples often contain less accurate annotations. To evaluate this factor, we inject different magnitudes of noise in labels to explore their impacts. 

\subsection{Dataset Attributes}
\label{single-dataset}

Different datasets may exhibit different attributes, which are critical for the model performance. To easily analyze their impacts, we use each dataset from our collection to train the HMR model, and test its performance. Table~\ref{table-singleds} summarizes the attributes and the corresponding performance. 

\input{Tables/single-dataset}

\textbf{Non-critical attributes}.
\citet{Joo2021} suggested that there exists an indoor-outdoor domain gap, where models trained on 
%outdoor datasets (e.g., COCO and MPII) do not perform well on indoor test datasets (H36M), and models trained on indoor datasets (e.g., H36M) has lower accuracy on outdoor test datasets (3DPW).
outdoor datasets do not perform well on indoor test datasets, and vice versa.
% \textit{However, our comprehensive benchmarks indicate this conclusion is too broad a generalization.} 
However, our comprehensive benchmarks reveal that not all datasets' performance can be explained by the indoor-outdoor domain gap, calling for a more careful analysis of underlying factors.
For instance, several notable indoor training datasets (\textit{e.g.}, PROX, MuCo-3DHP) outperform many outdoor datasets, and result in high-performing models on the outdoor 3DPW test dataset.
%: PROX and MuCo-3DHP achieve PA-MPJPE (\(mm\)) of 84.69 and 78.05 respectively. 
Similarly, we observe that some indoor training datasets (\textit{e.g.}, MPI-INF-3DHP, 3DOH50K) give a really poor performance on the indoor H36M test dataset, as shown in the appendix. In addition, we find weak correlations between the number of data points and model performance. For instance, COCO with 10x fewer data points outperforms H36M \citep{Ionescu2014} on the 3DPW test set. 

\textbf{Critical attributes.}
There are some attributes that can heavily impact the model performance, such as human poses, body shape (height, limb length), scenes, lighting, occlusion (self, people, environment), annotation types (2D/3D keypoints, SMPL) and camera characteristics (angles) \citep{Patel2021, Cai2021, Tian2022, Rapczynski2021, Joo2021, cai2020messytable}. High similarities of these attributes between the training and test datasets can yield better performance.
%
% \lei{What does 'collection methods' mean here?}
% As there is little information of the subjects' characteristics, action diversity, camera placement and scenes in the considered datasets, these four attributes could be a proxy for them.

To validate these, we adopt a well-trained HMR model to estimate the distributions of four attributes: 1) pose \( \theta \in R^{69}\), 2) shape \( \beta \in R^{10}\) and 3) camera translation \(t^{c} \in R^{3}\) obtained from the head, and 4) features \( f \in R^{2048}\) obtained from the ResNet-50 backbone. Fig.~\ref{pca-h36m-coco} visualizes the results with the UMAP dimension reduction technique \cite{mcinnes2018umap} for four selected datasets: COCO, 3DPW, H36M and MPI-INF-3DHP. 
We have the following observations. First, COCO has a large variety of these attributes, which considerably overlap with those of 3DPW. This explains why training with COCO gives satisfactory performance on 3DPW. Second, H36M lacks diversity in poses (Fig. \ref{pca-h36m-coco}a) and has distinctly different distributions of features (Fig. \ref{pca-h36m-coco}d) and shape (Fig. \ref{pca-h36m-coco}b) from 3DPW, possibly due to the limited number of subjects (9) and scenes (1) (Table \ref{table-singleds}). In addition, H36M's shape and camera distribution differ from MPI-INF-3DHP.
% We also observe dissimilar distributions of body shape and camera translation between MPI-INF-3DHP and H36M. 
Therefore, training with either 3DPW or MPI-INF-3DHP has poor performance on H36M. 
%Actually, only the H36M-train set yields good performance on the H36M-test set. 
H36M benchmarks and extra visualization of the attribute distributions for other datasets (Figs.~\ref{pca-pose} - \ref{pca-features}) can be found in the appendix.


% In COCO, the diverse distribution of the four attributes, and considerable overlap with those of 3DPW's . H36M and MPI-INF-3DHP has a distinctly different distributions of beta, pose, camera and backbone features with 3DPW-test and COCO and each other.

% \lei{Will we explain more details about the adopted attributes in appendix? For example, it is not quite sure how to get backbone features here.}

\input{Figs/pca-h36m-coco}

% In some datasets, people often appear under occlusion either due to self-overlapping body parts, close contact with other persons, or interactions with the environment \citep{Patel2021}. Person-person or person-object occlusion can be a more important factor that predominates the background. This can be observed from two cases (Fig. \ref{occlusion} in the appendix). (1) MUCO-3DHP is a dataset created through compositing MPI-INF-3DHP with the inter-person occlusion. From Table~\ref{table-singleds}, we observe that the HMR model trained with MuCo-3DHP has better performance than that with MPI-INF-3DHP (78.05 versus 107.15 in PA-MPJPE (\(mm\))). (2) PROX, despite being the only indoor 2D keypoint dataset, gives the best performance compared with other outdoor 2D keypoint datasets with the PA-MPJPE of 84.69 (\(mm\)) on 3DPW. PROX contains numerous instances of people interacting with the indoor furniture (Fig. \ref{occlusion}), which can improve the model performance. 


Notably, the indoor datasets that perform well on outdoor 3DPW benchmarks are designed with considerable person-person (MuCo-3DHP) and person-object occlusion (PROX) (Fig. \ref{occlusion} in the appendix). This suggests that occlusion can be a more important factor that predominates the background (see Appendix \ref{occ-analysis} for more details).


\input{Tables/eft-fittings}
To demonstrate the importance of the SMPL fitting mechanism, we compare EFT datasets with and without SMPL annotation, as shown in Table~\ref{table-eft}.
%compares the model performance with and without the fittings. 
We observe that EFT fittings can reduce the PA-MPJPE by over 20 \(mm\) for different datasets. This is consistent with the findings from \cite{Joo2021,Cai2021} that SMPL parameters ($\theta$ and $\beta$) provide stronger supervision signals compared to 2D and 3D keypoints. \citet{Cai2021} put forward the reason that strong supervision initiates the gradient flow that reaches the learnable SMPL parameters in the shortest possible route.



\begin{tcolorbox}[left=1mm, right=1mm, top=0.5mm, bottom=0.5mm, arc=1mm]
\textbf{Remark \#1:} The indoor/outdoor settings or number of data points are not strong indicators for the model performance. Some attributes (e.g., human pose and shape, camera characteristics, backbone features) are more critical, and having high diversities (leading to considerable overlap between the training and test sets distributions) can give more satisfactory results. Occlusion (person-person or person-object) and SMPL fittings can also help boost recovery accuracy. 
\end{tcolorbox}
%\vspace{-20pt}

\subsection{Combination of Multiple Datasets}

It is a common practice to train the mesh recovery model with multiple datasets of different domains and annotation types. Past works select the datasets empirically. We argue that different combinations of datasets can lead to a vast fluctuation in performance. We explore their impacts from two directions. 

\input{Tables/multi-datasets}

\textbf{Selection of datasets.}
We first evaluate different combinations of training datasets, as shown in Table \ref{table-multids}. Particularly, \emph{Mix 2} follows the selection in DSR \citep{Dwivedi2022} and EFT \cite{Joo2021} while \emph{Mix 6} follows that in PARE \citep{Kocabas2021}. We have several observations. First, the selection of the training sets has high impacts on the model performance, even more critical than the training algorithms. For instance, for \textit{Mix 2}, we obtain a PA-MPJPE of 55.98 \(mm\) using the HMR base model, while DSR and EFT report 54.1 \(mm\) and 54.7 \(mm\) respectively, with more advanced algorithms. The performance difference is minor compared to that with different combinations of datasets. Similarly, for \textit{Mix 6}, our HMR base model gets 55.47 \(mm\) whereas PARE reports 52.3 \(mm\). We observe that some prior works compare their model performance with algorithms trained on vastly different dataset mixes, which is arguably unfair. %This is not to diminish the efficacy of the algorithms, but to highlight that 
The lack of a defined and consistent combination of training datasets hinders the direct comparison of different algorithms' performance. Through our benchmarking, we provide the community with new baselines on some of the commonly used dataset combinations.
%
% \lei{It seems that the label "table-multids" has been used both in auto\_partition.tex and multi-dataset.tex table, thus Table 12 has been referred, instead of Table 4.}

Second, it is not necessary to include more datasets. From Table \ref{table-multids}, we observe that \emph{Mix 10} does not perform as well as other mixes with fewer datasets. Involving more datasets could harm the model accuracy. It is recommended to select the optimal combination of datasets rather than prioritizing the quantity. For instance, we discover that the involvement of EFT (especially EFT-COCO) datasets can boost the performance, which should be strongly considered as the baselines (Table \ref{table-multids}). 


\textbf{Dataset contributions.}
In addition to the selection of datasets, the relative contribution of each dataset in the combination is also important. Unfortunately, no prior works consider this factor. Basically, there are two approaches to adjust the dataset contribution. The first one is to set the partitions (i.e., probability that a dataset is ``seen'' during training) of these datasets with pre-defined ratios \citep{Kanazawa2017}. The second is to maintain the same partition and reweight samples from different datasets, similar to prior methods of weighting valuable samples \citep{Ren2018, Shu2019}. Table \ref{table-weighting} shows the model performance with different contribution configurations using 6 datasets in \citep{Kanazawa2017}. Our observations include: (1) Setting different contributions for different datasets can indeed alter the model performance. A careful configuration can bring a rather large improvement. It is important to increase the contributions of critical datasets that can benefit the training (e.g., COCO in our case). (2) Under the same contribution configurations, the approach of directly altering the partitions is more effective than reweighting the samples. 

% \vspace{-5}
\vspace{-3pt}
\begin{tcolorbox}[left=1mm, right=1mm, top=0.5mm, bottom=0.5mm, arc=1mm]
\textbf{Remark \#2:} The selection of datasets and their relative contributions are important factors to determine the model performance. To fairly evaluate and compare the impact of other factors (e.g., training algorithms), it is crucial to keep the same dataset combination configuration, which is usually ignored by prior works. To get a good baseline model, it is suggested to adopt more critical datasets and increase their contribution during training. 
\end{tcolorbox}
% \vspace{-5}
\input{Tables/partition-weighting}

\subsection{Annotation Quality}
Many algorithms use pseudo-annotations during training (Table \ref{Dataset-mixes} in the appendix). We assess how the annotation quality affects training. To this end, we generate datasets with controlled noise to reflect different magnitudes of corruption in real scenarios. We investigate the following aspects. 

\input{Figs/noise-results}

\textbf{Proportion of noisy samples.}
 We inject noise to different ratios of samples. We consider two scenarios: (1) only SMPL annotations is noisy, which might occur when challenging poses are wrongly fitted; (2) both keypoints and SMPL annotations are noisy as incorrect keypoint estimation leads to erroneous fittings \citep{Joo2021} (Fig. \ref{noise-keypoints-vis} in the appendix).

%  We inject noise to different ratios of samples. Particularly, (1) challenging poses could be incorrectly estimated. So we simulate the scenario where different proportions of samples contain corrupted SMPL annotations. (2) It is discovered that incorrect keypoint estimations lead to a portion of erroneous SPIN fittings. Since the fitting methods depend on keypoints accuracy \citep{Joo2021}, we simulate the scenario where a portion of samples contain both noisy keypoints and SMPL (Fig. \ref{noise-keypoints-vis} in the appendix).
 

Fig. \ref{proportion-noise}a shows the model performance on the 3DPW test set with different ratios of noisy samples in the above two scenarios. For scenario (1), the errors remain low under small portions of noisy SMPL annotations (<50\%). The trained model can generalize and learn with such noisy samples. When the amount of noisy SMPL annotations overwhelms the clean ones, the errors increase sharply. For scenario (2), when we add noisy keypoints on top of noisy SMPL, we obtain large increments in the recovery errors. It also increases significantly with more than 50\% noisy samples. A plausible reason is that when there are only noisy SMPL annotations, the clean keypoints can still provide supervision to keep errors low. However, when both keypoints and SMPL are noisy, the errors are dire. 


\textbf{Scale and location of noise.}
We further consider two more scenarios about the controlled noise (Fig. \ref{noise-vis} in the appendix). (1) We inject noise to the SMPL of all poses and vary its scales (i.e., standard deviation). The generated poses are still realistic. (2) We observe that fitted poses of certain body parts (i.e. feet and hand) tend to be less accurate in existing fittings. We simulate cases for wrongly fitted body parts by replacing a percentage of pose parameters (body parts) with random noise. 


Fig. \ref{proportion-noise}b shows the model performance, where we add noise of different standard deviations to all pose parameters (scenario 1), or totally random noise to different ratios of the pose parameters (scenario 2). When we increase the noise scale, the errors increase slightly and remain low (<70\%). However, when a portion of body part is replaced with random noise, errors increase by a large margin. This shows that clean SMPL annotations are important, but slightly noisy SMPL within realistic realms still helps training. SMPL fittings should be reasonably accurate, but need not be perfect. 
%
% \lei{Fig. \ref{proportion-noise} does not have (a)(b); not very sure the correspondence between legend(Std, Pose) and Scenario(1, 2) in right figure}
\vspace{-5pt}
\begin{tcolorbox}[left=1mm, right=1mm, top=0.5mm, bottom=0.5mm, arc=1mm]
\textbf{Remark \#3:} Noisy data samples can harm the model performance, especially when the ratio of samples is higher, or both the SMPL annotation and keypoints are compromised. Slightly noisy SMPL still helps training.
\end{tcolorbox}





==> Sections/0304_combine_training_strategy.tex <==
\section{Benchmarking Training Strategies}
\label{training-strategies}
% %We further consider different training strategies that can enhance the model performance. 
\subsection{Augmentation}
% PASCAL-VOC \citep{Everingham10} 
%\textbf{Augmentation.}
Various augmentation methods have been adopted for mesh recovery. SPIN  \citep{Kocabas2021} utilized rotation, flip and color noising. PARE \citep{Kocabas2021} and BMP \citep{Zanfir2021} added synthetic occlusion by compositing a random nonhuman object to the image. BMP \citep{Zhang2021} made it keypoint-aware by occluding randomly selected keypoints. \citet{Georgakis2020} controlled the extent of occlusion by varying the pattern (oriented bars, circles, rectangles) size. \citet{Mehta2018} created inter-person overlap in the datasets. Other than occlusion, crop augmentation has also been applied to better reconstruct highly truncated people \citep{Rockwell2020,Joo2021,Kocabas2021}. Augmentation has also been used to bridge the synthetic-to-real domain gap \citep{Pavlakos, Doersch2019, Xu2019, Sengupta2020}. However, the above studies adopt different configurations and benchmarks, and it is hard to get general conclusions about the effect of different augmentations.

% However, the above studies adopt different configurations and benchmarks, and it is hard to get general conclusions about the effect of different augmentations.

% \citet{Sengupta2020} added shape and proxy representation augmentation.

We systematically evaluate and compare 9 image-based augmentations over different training and test datasets. Specifically, we re-implement common augmentation techniques in prior mesh recovery works, such as random occlusion (or hard erasing) \citep{Li2021,Zhong2020}, synthetic occlusion \citep{Kocabas2021} and crop augmentation \citep{Kocabas2021, Joo2021}. 
%\citet{Georgakis2020} investigated the robustness of a model under various degrees of random occlusion by varying the size of the occlusion pattern. As we are more concerned with investigating different types of occlusion instead of the extent of occlusion, we adopted random occlusion following \citet{Li2021, Zhong2020} instead as \citet{Georgakis2020} is too fine-grained and beyond the scope of our investigation. 
Besides, we also adopt popular augmentations from person reidentification and pose estimation tasks, such as soft erasing \citep{chen2021benchmarks}, self-mixing \citep{chen2021benchmarks}, photometric distortion \citep{buslaev2020albumentations}, coarse and grid dropouts \citep{buslaev2020albumentations}. Fig. \ref{aug} visualizes the augmented results by different techniques.  


\input{Figs/augmentation}
\input{Tables/augmentation}




We consider two individual training datasets with distinct characteristics: the indoor H36M set and outdoor EFT-COCO. We apply different augmentations to both datasets to train the HMR models, before evaluating them on five test datasets: 3DPW, EFT-LSPET, EFT-OCHuman, EFT-COCO and H36M. Table \ref{aug-h36m-coco} reveals the distinct effects of augmentation on these two training datasets. (1) For H36M, almost all the augmentations help the trained model achieve lower errors across outdoor test sets, and self-mixing is the most effective solution. This implies that augmentation can help bridge the indoor-outdoor domain gap and prevent overfitting. In the appendix, Fig. \ref{aug-h36m-perf} compares the training curves with and without augmentation to confirm this conclusion. Fig. \ref{aug-camera-h36m-coco} shows the distribution of camera features after applying self-mixing, which overlaps substantially with the predicted features obtained from a robust model that performs well on 3DPW-test. (2) For EFT-COCO, we observe that robust augmentations seldom improve the model performance on the test sets of 3DPW, EFT-LSPET and EFT-OCHuman, with the exception of EFT-COCO-val. This is consistent with the findings in \citet{Joo2021}: EFT-COCO-train already includes many robust samples with severe occlusions. Adding more extensive augmentation can harm the model performance. 

%In our experiments, photometric distortion seems to be the only augmentation that consistently improves performance across all benchmarks (Table \ref{aug-h36m-coco}). Similar to \citet{Joo2021}, we find that evaluation on internet videos showcases the usefulness of augmentations in tackling difficult in-the-wild cases, even though they might not have improved 3DPW benchmarks.


%Training without augmentation increases the indoor-outdoor domain gap, as evidenced from the increasing errors (PA-MPJPE) on 3DPW throughout the training episode (Fig. \ref{aug-h36m-perf}). Addition of augmentation helps to close the indoor-outdoor domain gap, achieve lower errors and prevent overfitting (Fig. \ref{aug-h36m-perf}). Amongst the augmentations, self-mixing seems to be the most helpful for H36M (Table \ref{aug-h36m-coco}). This is also evident from Fig. \ref{aug-camera-h36m-coco} where the distribution of camera features after applying self-mixing overlaps substantially with the predicted features obtained from a robust model that performs well on 3DPW-test.



%Varying effectiveness was reported from applying different augmentations (see section \ref{related-works-training-strategy}), prompting us to analyse the effect of augmentation on individual datasets with respect to their underlying feature distributions. As seen from Table \ref{aug-h36m-coco}, almost all augmentations help HMR trained on H36M to achieve lower errors across several outdoor benchmarks such as 3DPW-test, EFT-LSPET-test, EFT-OCHuman-test and EFT-COCO-val. Training without augmentation increases the indoor-outdoor domain gap, as evidenced from the increasing errors (PA-MPJPE) on 3DPW throughout the training episode (Fig. \ref{aug-h36m-perf}). Addition of augmentation helps to close the indoor-outdoor domain gap, achieve lower errors and prevent overfitting (Fig. \ref{aug-h36m-perf}). Amongst the augmentations, self-mixing seems to be the most helpful for H36M (Table \ref{aug-h36m-coco}). This is also evident from Fig. \ref{aug-camera-h36m-coco} where the distribution of camera features after applying self-mixing overlaps substantially with the predicted features obtained from a robust model that performs well on 3DPW-test.

%In contrast, applying robust augmentations to EFT-COCO seldom improve nor attain marginal improvements for benchmarks on 3DPW-Test, EFT-LSPET-test and EFT-OCHuman-test, with the exception of EFT-COCO-Val (Fig. \ref{aug-h36m-coco}). Our findings concur with that of \citet{Joo2021}, who purported that EFT-COCO already includes many robust samples with severe occlusions \citep{Joo2021}. In our experiments, photometric distortion seems to be the only augmentation that consistently improves performance across all benchmarks (Table \ref{aug-h36m-coco}). Similar to \citet{Joo2021}, we find that evaluation on internet videos showcases the usefulness of augmentations in tackling difficult in-the-wild cases, even though they might not have improved 3DPW benchmarks.
\vspace{-5pt}
\begin{tcolorbox}[left=1mm, right=1mm, top=0.5mm, bottom=0.5mm, arc=1mm]
\textbf{Remark \#5:} The effect of data augmentations highly depends on the characteristics of the training dataset. Their benefits are more obvious when the training sets contain less diverse and robust samples. 
%When the training samples are more robust with similar feature distributions as the test set, applying augmentation brings less positive effects or even compromises the model performance. 
When combining multiple datasets during training, we can selectively run data augmentations to different datasets based on their characteristics. 
\end{tcolorbox}




%When combining multiple datasets during training, certain augmentations might bring about greater benefits on selected datasets but less so on others. This might be explained by the differences in characteristics of each dataset (Fig. \ref{pca-h36m-coco}), where the distribution of pose, beta, camera and backbone features of EFT-COCO already overlaps considerably with the distributions in 3DPW-test. Therefore, applying robust augmentation has a less pronounced effect on EFT-COCO than H36M (Fig. \ref{aug-perf}). 


\subsection{Training Loss}
%Prior works commonly train the HMR models with a mixture of losses: regression of the keypoints and SMPL parameters are supervised with the MSE loss, while the vertex is learned with the L1 loss. We experiment with alternative settings where a unified loss (either MSE or L1) is applied to all the parameters, which gives us unexpected good results. 
% We experiment with alternative settings where a different loss is applied.
Prior works commonly adopt the MSE loss in pose estimation involving keypoints \citep{Feng2019, Munea2020}. In HMR, regression of keypoints and SMPL parameters are supervised with the MSE loss. We experiment with alternative settings where a different loss is applied. As the L1 loss function measures the magnitude of the error but does not consider the direction, it is insensitive to outliers. Under certain assumptions, \citet{Ghosh2015} theoretically demonstrated that L1 can be robust against noisy labels. Inspired by this, we use L1 in place of MSE loss for the regression of keypoints and SMPL parameters in HMR. We note that this replacement can improve the model from two directions. First, it helps to tackle noisy samples. Fig. \ref{l1-noise} compares the HMR model performance with MSE and L1 loss functions under different scales of SMPL noise, and proportions of noisy keypoints and SMPL annotations, respectively. We find that L1 loss can make the model more robust to noise. 

\input{Tables/l1-multi-datasets}

Second, L1 loss improves model performance under the multi-dataset setting. Table \ref{l1-multids} compares the performance with and without L1 loss trained on different dataset combinations. We observe that L1 loss can bring significant performance gains. In particular, applying L1 loss to the dataset configurations in SPIN \citep{Kolotouros2019} reduces the errors from 64.55 \(mm\) to 58.20 \(mm\). We also note that the L1 loss gain becomes smaller when the dataset selection is more optimal (\emph{Mix 2, 6, 8}). 

\begin{tcolorbox}[left=1mm, right=1mm, top=0.5mm, bottom=0.5mm, arc=1mm]
\textbf{Remark \#6:} Prior works adopt MSE loss for regression of keypoints and SMPL parameters. Using L1 loss instead can not only improve the model's robustness against noisy samples, but also enhance the model performance, especially when the selected datasets are not optimal.
\end{tcolorbox}

%Taking inspiration from \citet{Ghosh2015}, using L1 in place of MSE losses helped to tackle noise and kept errors low (<70 PA-MPJPE) under acceptable levels of noise (Fig. \ref{l1-noise}a) and proportion (<50\%) of noisy keypoints and SMPL annotations(Fig. \ref{l1-noise}b). In our case, the success of training with L1 loss is unexpected, as L1 loss trains well on a relatively deep neural network with multiple heads contrary to findings by \citet{Zhang2018}. 

%Other than tackling noise, L1 improves performance on multi-dataset benchmarks (Table \ref{l1-multids}). Significant improvements gains can be achieved from adopting L1 loss when performance has saturated (Table \ref{l1-multids}). In particular, applying L1 loss to SPIN's \citep{Kolotouros2019} selection of datasets reduced errors to 58.19, outperforming SPIN \citep{Kolotouros2019}, an optimisation-based method. However, we note that when benchmarks are saturated (50+ PA-MPJPE), minor improvements can be made by applying L1 loss (Table \ref{l1-multids}).



%A less typical loss is the Mean Absolute Error (MAE) or L1 loss function \citep{Munea2020}, calculated by taking the mean of the absolute differences between true and predicted values. As L1 loss function measures the magnitude of the error but does not consider the direction, it is insensitive to outliers. Under certain assumptions, \citet{Ghosh2015} theoretically demonstrated that L1 can be robust against noisy labels. However, this was contested by \citet{Zhang2018} who  showed that L1 loss can be difficult to optimize and might end up harming training performance. This flaw is exacerbated when applying MAE on deep neural networks and complicated datasets \citep{Zhang2018}. L1 has also been seldomly used in deep networks as it is difficult to regress precisely \citep{Munea2020}. 


%Taking inspiration from \citet{Ghosh2015}, using L1 in place of MSE losses helped to tackle noise and kept errors low (<70 PA-MPJPE) under acceptable levels of noise (Fig. \ref{l1-noise}a) and proportion (<50\%) of noisy keypoints and SMPL annotations(Fig. \ref{l1-noise}b). In our case, the success of training with L1 loss is unexpected, as L1 loss trains well on a relatively deep neural network with multiple heads contrary to findings by \citet{Zhang2018}. 

%Other than tackling noise, L1 improves performance on multi-dataset benchmarks (Table \ref{l1-multids}). Significant improvements gains can be achieved from adopting L1 loss when performance has saturated (Table \ref{l1-multids}). In particular, applying L1 loss to SPIN's \citep{Kolotouros2019} selection of datasets reduced errors to 58.19, outperforming SPIN \citep{Kolotouros2019}, an optimisation-based method. However, we note that when benchmarks are saturated (50+ PA-MPJPE), minor improvements can be made by applying L1 loss (Table \ref{l1-multids}).


\input{Figs/l1-results}

==> Sections/06_conclusion.tex <==
% \section{Conclusion}

%  unifying a common training set
%Training with multiple datasets is a setting rather unique to mesh recovery works. Many works have exploited different dataset selection and backbones to achieve performance on benchmarks. As of our knowledge, this work is the first large-scale benchmarking of single and mixed datasets for mesh recovery tasks. We believe that providing a strong baseline on several commonly used partitions using HMR \citep{Kanazawa2017} could encourage unbiased comparisons. We identified that weight initialisation and using L1 loss is essential for improving performance. Further, we investigate why different studies reported contrasting effectiveness of augmentations and compared the feature distributions of different datasets. We hope that these insights could drive innovation in future works. 

% \subsection{Limitations}
%\paragraph{Limitations}
%All of our benchmarks are performed with HMR \citep{Kanazawa2017}. Due to time constraints, we did not evaluate our findings on other algorithms. 

==> Tables/auto_partition.tex <==
\begin{wraptable}{r}{0.63\textwidth}
%\vspace{-10pt}
\centering
\tiny
\caption{Performance (PA-MPJPE in \(mm\)) of the HMR model on the 3DPW test set when trained without optimizer, and with Bayes or Policy Gradients (PG) as optimizers.}
\label{auto-partitions}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}c|l|ccc@{}}
\Xhline{1pt}
\textbf{Mix}           & \textbf{Datasets}                                          & \textbf{Original}& \textbf{Bayes}  & \textbf{PG}\\ \Xhline{1pt}
1 & H36M, MI, COCO                       & 66.14   &65.14 &  62.15                            \\
2 & H36M, MI, EFT-COCO                       & 55.98    & 56.29 & 54.94                             \\
5 & H36M, MI, COCO, LSP, LSPET, MPII         & 64.55 &62.77 &  62.95                               \\6 & EFT-[COCO, MPII, LSPET], SPIN-MI, H36M  & 55.47  & 56.51 &   56.66                           \\  \Xhline{1pt}    
\end{tabular}
\end{adjustbox}
\end{wraptable}


==> Tables/combine.tex <==
% \begin{table}
\begin{wraptable}{r}{0.6\textwidth}
\vspace{-12pt}
\tiny
\caption{\small \textbf{Our identified optimal baseline models with the performance on the 3DPW test set.} Abbreviations for the datasets - Human3.6M \citep{Ionescu2014}: H36M, MPI-INF-3DHP \citep{Mehta2017}: MI, MuCo-3DHP \citep{Mehta2018}: MuCo, PoseTrack \citep{Andriluka2018}: PT, OCHuman \citep{Zhang2019}: OCH}
\vspace{-5pt}
\label{combine-results}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}c|l|c|c@{}}
\Xhline{1pt}
\multicolumn{1}{c|}{\textbf{Algorithm}} & \multicolumn{1}{c|}{\textbf{Dataset}}                         &\textbf{Backbone}  & \multicolumn{1}{c}{\textbf{PA-MPJPE$\downarrow$}} \\ \Xhline{1pt}
PARE \citep{Kocabas2021} & EFT-[COCO, LSPET, MPII], H36M, SPIN-MI               & HrNet-W32     & 50.90 \\
Ours & EFT-[COCO, LSPET, MPII], H36M-Aug, SPIN-MI               & HrNet-W32     & 47.68  \\ \hline
SPIN \citep{Kolotouros2019} & H36M, MI, COCO, LSP, LSPET, MPII & ResNet-50         & 59.2                  \\
HMR \citep{Kanazawa2017} & H36M, MI, COCO, LSP, LSPET, MPII & ResNet-50         & 76.7                 \\
Ours & H36M, MI, COCO, LSP, LSPET, MPII & ResNet-50         & 51.66    \\
Ours & H36M, MI, COCO, LSP, LSPET, MPII & Twin-SVT-B               & 48.77                        \\  \hline
Ours &  H36M, MI, COCO, LSP, LSPET, MPII & HrNet-W32         & 49.18                        \\
Ours & H36M-Aug, MI, COCO, LSP, LSPET, MPII & Twin-SVT-B           & 47.70      \\
Ours & EFT-[COCO, LSPET, MPII], H36M, SPIN-MI               & Twin-SVT-B     & 47.31 \\
Ours & H36M, MI, EFT-COCO               & HrNet-W32               & 48.08 \\ 
Ours & H36M, MI, EFT-COCO               & Twin-SVT-B               & 48.27 \\
Ours & H36M, MuCo, EFT-COCO               & Twin-SVT-B              & 47.92  \\
Ours & EFT-[COCO, LSPET, PT, OCH] H36M, MI & Twin-SVT-B                 & 49.33  
 \\ \Xhline{1pt}
\end{tabular}
% \end{table}
\end{adjustbox}
\vspace{-8pt}
\end{wraptable}



% % WITH H36M results
% % \begin{table}
% \begin{wraptable}{r}{0.5\textwidth}
% \vspace{-10pt}
% \tiny
% \caption{Optimal baseline models with the configurations and performance (PA-MPJPE in \(mm)\)}
% \label{combine-results}
% \begin{adjustbox}{max width=\linewidth}
% \begin{tabular}{@{}c|l|c|cc@{}}
% \Xhline{1pt}
% \multicolumn{1}{c}{\textbf{Algorithms}} & \multicolumn{1}{c|}{\textbf{Dataset \footnote{Short forms used - Human3.6M \citep{Ionescu2014}: H36M, MPI-INF-3DHP \citep{Mehta2017}: MI, MuCo-3DHP \citep{Mehta2018}: MuCo, PoseTrack \citep{Andriluka2018}: PT, OCHuman \citep{Zhang2019}: OCH}}}                         &\textbf{Backbone}  & \multicolumn{1}{c}{\textbf{3DPW$\downarrow$}} & \multicolumn{1}{c}{\textbf{H36M$\downarrow$}} \\ \Xhline{1pt}
% SPIN & H36M, MI, COCO, LSP, LSPET, MPII & ResNet-50         & 59.2   & 41.1                           \\
% HMR & H36M, MI, COCO, LSP, LSPET, MPII & ResNet-50         & 76.7   & 56.8                           \\
% Ours & H36M-Aug, MI, COCO, LSP, LSPET, MPII & ResNet-50         & 51.96   & TBC \\
% Ours & H36M-Aug, MI, COCO, LSP, LSPET, MPII & ResNet-50         & 51.87   & TBC                           \\
% Ours &  H36M, MI, COCO, LSP, LSPET, MPII & HrNet-W32         & 49.18   & 46.49                           \\
% Ours & H36M, MI, COCO, LSP, LSPET, MPII & Twin-SVT-B               & 48.77  &43.07                              \\
% Ours & H36M-Aug, MI, COCO, LSP, LSPET, MPII & Twin-SVT-B           & 47.70    & 42.73                             \\
% PARE & EFT-[COCO, LSPET, MPII], H36M, SPIN-MI               & HrNet-W32     & 50.9  & - \\
% Ours & EFT-[COCO, LSPET, MPII], H36M-Aug, SPIN-MI               & HrNet-W32     & 47.68  & 53.95 \\
% Ours & EFT-[COCO, LSPET, MPII], H36M, SPIN-MI               & Twin-SVT-B     & 47.31  & 43.33 \\
% Ours & H36M, MI, EFT-COCO               & HrNet-W32               & 48.08   & 46.00 \\ 
% Ours & H36M, MI, EFT-COCO               & Twin-SVT-B               & 48.27  & 42.97  \\
% Ours & H36M, MuCo, EFT-COCO               & Twin-SVT-B              & 47.92  & 46.90  \\
% Ours & EFT-[COCO, LSPET, PT, OCH] H36M, MI & Twin-SVT-B                 & 49.33 & 46.55 
%  \\ \Xhline{1pt}
% \end{tabular}
% % \end{table}
% \end{adjustbox}
% \end{wraptable}

==> Tables/dataset-mixes.tex <==
\begin{table}[h!]
\tiny
\caption{\small \textbf{Summary of the datasets used in various mesh recovery methods and their reported performance (PA-MPJPE in \(mm\)) on 3DPW and H36M datasets}. Abbreviation for the dataset - Human3.6M \citep{Ionescu2014}: H36M, MPI-INF-3DHP \citep{Mehta2017}: MI, MuCo-3DHP \citep{Mehta2018}: MuCo, PoseTrack \citep{Andriluka2018}: PT, OCHuman \citep{Zhang2019}: OCH. 3DPW \emph{Protocol 2} (P2) refers to the evaluation (PA-MPJPE) on 3DPW test set without training on 3DPW train set while \emph{Protocol 1} (P1) includes fine-tuning on 3DPW train set. We use the notation {[}*{]}$_{\textrm{EFT/ SPIN/ SMPLify-X}}$ to denote datasets with EFT, SPIN or SMPLify-X fittings.}
\label{Dataset-mixes}
\begin{tabular}{@{}lllll@{}}
\toprule
Method                  & Datasets used                                                                                                     & 3DPW (P2)$\downarrow$ & 3DPW (P1)$\downarrow$ & H36M$\downarrow$ \\ \midrule
HMR \citep{Kanazawa2017}                     & H36M, MI, COCO, LSP, LSPET, MPII                                                                        & 76.7      & -         & 56.8 \\
NBF \citep{Omran2018}                     & H36M, UP-3D,  HumanEva-I                                                                                           & -         & -         & 59.9 \\
GraphCMR \citep{Kolotouros2019b}                & H36M, UP-3D, COCO, LSP, MPII                                                                                      & 70.2      & -         & -    \\
HoloPose \citep{Guler2019}                & H36M, MPII, {[COCO]}$_{\textrm{Densepose}}$                                                                                 & -         & -         & 46.5 \\
SPIN \citep{Kolotouros2019}                    & H36M, {[MI]}$_{\textrm{SPIN}}$, COCO, LSP, LSPET, MPII                                                            & 59.2      & -         & 41.1 \\
\citet{Jiang2020} & H36M, MI, PT, LSP, LSPET, MPII, COCO                                                             &           &           & 52.7 \\
\citet{Zhang2020}                   & H36M, {[COCO]}$_{\textrm{Densepose}}$, UP3D, [LSP, LSPET, MPII, COCO]$_{\textrm{SPIN}}$                                          &           &           & 41.7 \\
Pose2Mesh \citep{Choi2020}               & MuCo, {[H36M]}$_{\textrm{SMPLify-X}}$, COCO, Freihand                                                                  & 58.9      &           & 47   \\
HKMR \citep{Georgakis2020}                   & H36M, MI, COCO, LSP, LSPET, MPII                                                                        &           &           & 43.2 \\
I2L-MeshNet \citep{Moon2020}             & MuCo, {[H36M]}$_{\textrm{SMPLify-X}}$, COCO, Freihand                                                                  & 57.7      &           & 41.1 \\
DaNet \citep{Zhang2022}                   & H36M, {[COCO]}$_{\textrm{Densepose}}$, UP3D, {[}LSP, LSPET, MPII, COCO{]}$_{\textrm{SPIN}}$                                           & 54.8      &           & 40.5 \\
Pose2Pose \citep{Moon2022}              & MuCo, {[H36M]}$_{\textrm{SMPLify-X}}$, COCO-Wholebody, Freihand                                                        & 55.3      &           & 47.4 \\
HybrIK \citep{Li2021}                  & H36M, MI, COCO                                                                                          & 48.8      &           &      \\
METRO                 & H36M, UP-3D, MuCo, COCO, MPII, Freihand                                                                     &           & 47.9      & 36.7 \\
BMP \citep{Zhang2021}          & H36M, MI, MuCo, COCO, LSP, LSPET, PT, MPII                            & 63.8      &           & 51.3 \\
HUND \citep{Zanfir2021}                    & H36M, 3DPW, COCO-2017, OpenImages                                                                                 & 57.5      &           & 53   \\
EFT \citep{Joo2021}                    & {[}COCO, MPII, LSPET{]}$_{\textrm{EFT}}$                                                                                  & 54.2      & 52.2      &      \\
ProHMR\citep{Kolotouros2021}                  & H36M,  {[}MI, COCO, MPII{]}$_{\textrm{SPIN}}$                                                                       &           & 59.8      & 41.2 \\
DSR \citep{Dwivedi2022}                     & H36M, MI, {[}COCO{]}$_{\textrm{EFT}}$                                                                                & 54.1      & 51.7      &      \\
ROMP \citep{Sun2022}                    & H36M, UP-3D, [MI, COCO, MPII, LSP]$_{\textrm{SPIN}}$, AICH                                               & 54.9      & 62        &      \\
ROMP\citep{Sun2022}                     & H36M, UP-3D, [MI, COCO, MPII, LSP]$_{\textrm{SPIN}}$, AICH, PT, CrowdPose, MuCo, OH & 53.3      & 56.8      &      \\
Graphormer              & H36M, MuCo, UP-3D, COCO, MPII                                                                                & 45.6      &           & 34.5 \\
THUNDR \citep{Zanfir2022}                 & H36M, 3DPW, COCO-2017, OpenImages                                                                                 & 51.5      &           & 39.8 \\
PyMAF \citep{Zhang2021c}                  & H36M, {[MI]}$_{\textrm{SPIN}}$, COCO, LSP, LSPET, MPII                                                            & 58.9      & 51.2      & 40.5 \\
SPEC \citep{Kocabas2022}                    & Pano360, SPEC-SYN, SPEC-MTP, 3DPW, MI, H36M, {[}COCO, MPII, LSPET{]}$_{\textrm{EFT}}$                                     & 53.2      &           &      \\
PARE \citep{Kocabas2021} (ResNet-50)              & {[}COCO, MPII, LSPET{]}$_{\textrm{EFT}}$, MI, H36M                                                                 & 52.3      &           &      \\
PARE \citep{Kocabas2021} (HRNet-W32)        & {[}COCO, MPII, LSPET{]}$_{\textrm{EFT}}$, MI, H36M                                                                 & 50.9      & 46.5      &      \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/losses.tex <==
\begin{wraptable}{r}{0.37\textwidth}
\vspace{-10pt}
\centering
\tiny
\caption{Performance (PA-MPJPE in \(mm\)) of the HMR model using different losses.}
\label{l1-multids}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}c|cc@{}}
\Xhline{1pt}
\textbf{Losses}  & \textbf{3DPW} & \textbf{H36M}\\ \Xhline{1pt}
Mixed         & 64.55  & 46.47                               \\
All MSE     & 67.12  & -                        \\
All L1    & 58.20 & 49.61     \\           \Xhline{1pt}    
\end{tabular}
\end{adjustbox}
\end{wraptable}


==> Tables/multi-datasets.tex <==
\begin{wraptable}{r}{0.55\textwidth}
\vspace{-15pt}
\centering
\tiny
\caption{\small \textbf{HMR model performance when trained with different combinations of datasets.}}
\vspace{-5pt}
\label{table-multids}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}c|l|c@{}}
\Xhline{1pt}
\textbf{Mix}           & \multicolumn{1}{c|}{\textbf{Datasets}}                                          & \textbf{PA-MPJPE$\downarrow$} \\ \Xhline{1pt}
1 & H36M, MI, COCO                       & 66.14                      \\
2 & H36M, MI, EFT-COCO                       & 55.98                        \\
3 & H36M, MI, EFT-COCO, MPII                       & 56.12                          \\
4 & H36M, MuCo, EFT-COCO                       & 53.90                        \\
5 & H36M, MI, COCO, LSP, LSPET, MPII         & 64.55                         \\6 & EFT-[COCO, MPII, LSPET], SPIN-MI, H36M  & 55.47                    \\
% 7 & EFT-[COCO, MPII, LSPET], MuCo, H36M, PROX  & 55.27  &-                \\
7 & EFT-[COCO, MPII, LSPET], MuCo, H36M, PROX  & 53.44          \\ % different partition
8 & EFT-[COCO, PT, LSPET], MI, H36M  & 55.97  \\           
9 & EFT-[COCO, PT, LSPET, OCH], MI, H36M  & 55.59          \\ 
10 & PROX, MuCo, EFT-[COCO, PT, LSPET, OCH], UP-3D, MTP, Crowdpose  & 57.84           \\
11 & EFT-[COCO, MPII, LSPET], MuCo, H36M & 52.54      \\
\Xhline{1pt}    
\end{tabular}
\end{adjustbox}
\vspace{-10pt}
\end{wraptable}


==> Tables/single-dataset.tex <==

\begin{table}
\vspace{-17pt}
\centering
\tiny
\caption{\small \textbf{HMR model performance when trained on individual datasets.
For PROX and MuPoTs-3D, only 2D keypoints are used for training. P: person-person occlusion O: person-object occlusion.}} 
%* For these datasets, only 2D keypoints were used for training. Most models achieved convergence within 100 epochs but some required longer (we only managed to replicate the benchmark on EFT-COCO (58.63) similar to \citet{Joo2021} when trained for 200 epochs).  }
\label{table-singleds}
\begin{adjustbox}{max width=0.9\linewidth}
\begin{tabular}{@{}c|ccccccc|cc@{}}
\Xhline{1pt}
                    \textbf{Training dataset}    & \textbf{Annotation type}  & \textbf{Env.}   & \textbf{\# Samples} & \textbf{\# Subjects} & \textbf{\# Scenes} & \textbf{\# Cam} & \textbf{Occ.}            &   \textbf{PA-MPJPE$\downarrow$}  \\ \Xhline{1pt}
PROX \citep{Hassan2019} *                        & 2DKP             & Indoor                      & 88484                    & 11 & 12       & -       & O                            & 84.69                                                      \\
COCO-Wholebody \citep{Jin2020} & 2DKP             & Outdoor & 40055         & 40055 & -    & -       & -                                      & 85.27                                      \\
Instavariety \citep{Kanazawa2019}            & 2DKP             & Outdoor                         & 2187158       & >28272 & -   & -  & -                    & 88.93                                            \\
COCO \citep{Lin2014}                         & 2DKP             & Outdoor                         & 28344         & 28344 & -   & -    & -                          & 93.18                       \\
MuPoTs-3D \citep{Mehta2018} *  & 2DKP             & Outdoor                         & 20760             & 8 & -  & 12     & -                           & 95.83                          \\
LIP \citep{Gong2017}                      & 2DKP             & Outdoor                         & 25553              & 25553   & -   & -   & -                          & 96.47                            \\
MPII \citep{Andriluka2014}                     & 2DKP             & Outdoor                         & 14810         & 14810 & 3913  & -  & -                            & 98.18                                \\
Crowdpose \citep{Li2019}               & 2DKP             & Outdoor                         & 13927            & -  &-  & -      & P                   & 99.97                                  \\
Vlog People \citep{Kanazawa2019}                     & 2DKP             & Outdoor                         & 353306        & 798 &798   & -    & -                               & 100.38                             \\
PoseTrack (PT) \citep{Andriluka2018}                & 2DKP             & Outdoor                         & 5084          &550 &550    & -    & -                             & 105.30                         \\
LSP \citep{Johnson2010}                      & 2DKP             & Outdoor                         & 999           & 999 & -    & -       & -                                & 111.45                          \\
AI Challenger \citep{Wu2017}                      & 2DKP             & Outdoor                         & 378374        & - & -    & - & -                                & 111.66                    \\
LSPET \citep{Johnson2011}                     & 2DKP             & Outdoor                         & 9427       & 9427 & -    & -      & -                           & 112.26                      \\
Penn-Action \citep{Zhang2013}            & 2DKP             & Outdoor                         & 17443       & 2326      & 2326   & -    & -                        & 114.53                                     \\
OCHuman (OCH) \citep{Zhang2019}                  & 2DKP             & Outdoor                         & 10375    & 8110 & -   & -      & P,O                                   & 130.55                                             \\
MuCo-3DHP (MuCo) \citep{Mehta2018}               & 2DKP/ 3DKP       & Indoor                         & 482725         & 8 & -   & 14      & P                        & 78.05                                            \\
MPI-INF-3DHP (MI) \citep{Mehta2017}           & 2DKP/ 3DKP       & Indoor                         & 105274       & 8 & 1     & 14  & -                              & 107.15                     \\
3DOH50K (OH) \citep{Zhang2020}                 & 2DKP/ 3DKP       & Indoor                         & 50310        & -  & 1   & 6     & O                        & 114.48                                        \\
3D People \citep{Pumarola2019}                & 2DKP/ 3DKP       & Indoor                         & 1984640       & 80  & -   & 4 & -                               & 118.31                           \\
AGORA \citep{Patel2021}                    & 2DKP/ 3DKP/ SMPL & Indoor                         & 100015         & >350  & -  & -       & P,O                                & 88.65                      \\
SURREAL \citep{Varol2017}                  & 2DKP/ 3DKP/ SMPL & Indoor                         & 1605030       & 145  & 2607    & -    & -                              & 110.00                            \\
Human3.6M (H36M) \citep{Ionescu2014}                     & 2DKP/ 3DKP/ SMPL & Indoor                         & 312188       & 9  & 1     & 4    & -                          & 124.55                                           \\
EFT-COCO \citep{Joo2021}                & 2DKP/ SMPL       & Outdoor                         & 74834         & 74834 & -    & -     & -                             & 60.82                                    \\
EFT-COCO-part \citep{Joo2021}           & 2DKP/ SMPL       & Outdoor                         & 28062       & 28062 & -    & -               & -               & 67.81                                              \\
EFT-PoseTrack \citep{Joo2021}            & 2DKP/ SMPL       & Outdoor                         & 28457       & 550 & -     & -     & -                         & 75.17                                           \\
EFT-MPII \citep{Joo2021}                 & 2DKP/ SMPL       & Outdoor                         & 14667     & 3913 & -     & -     & -                               & 77.67                             \\
UP-3D \citep{Lassner2017}                    & 2DKP/ SMPL       & Outdoor                         & 7126        & 7126 & -   & -    & -                                & 86.92                                  \\
MTP \citep{Muller2021}                     & 2DKP/ SMPL       & Outdoor                         & 3187           & 3187 & -    & -      & -                            & 87.03                                        \\
EFT-OCHUMAN \citep{Joo2021}              & 2DKP/ SMPL       & Outdoor                         & 2495        & 2495 & -   & -       & P,O                              & 94.01                              \\
EFT-LSPET \citep{Joo2021}                & 2DKP/ SMPL       & Outdoor                         & 2946       & 2946 & -     & -               & -                & 100.53                             \\
3DPW \citep{VonMarcard2018}                    & SMPL             & Outdoor                         & 22735    & 7 & -   & -   & -                                & 89.36                \\ \Xhline{1pt}
\end{tabular}
\end{adjustbox}
\end{table}

==> Tables/single-dataset_w_h36m.tex <==

\begin{table}[!htb]
\tiny
\caption{\small \textbf{HMR model performance (PA-MPJPE in \(mm\)) on the 3DPW \citep{VonMarcard2018} and H36M\citep{Ionescu2014} test sets when trained on individual datasets. 
%For fair comparisons, all models are trained for 100 epochs. 
For PROX and MuPoTs-3D, only 2D keypoints are used for training. P: person-person occlusion O: person-object occlusion.}} 
%* For these datasets, only 2D keypoints were used for training. Most models achieved convergence within 100 epochs but some required longer (we only managed to replicate the benchmark on EFT-COCO (58.63) similar to \citet{Joo2021} when trained for 200 epochs).  }
\label{table-singleds-w-h36m}
\begin{tabular}{@{}c|ccccccc|cc@{}}
\Xhline{1pt}
                    \textbf{Training dataset}    & \textbf{Annotation type}  & \textbf{Env.}   & \textbf{\# Samples} & \textbf{\# Subjects} & \textbf{\# Scenes} & \textbf{\# Cam} & \textbf{Occ.}            &   \textbf{3DPW$\downarrow$} &  \textbf{H36M$\downarrow$} \\ \Xhline{1pt}
PROX \citep{Hassan2019} *                        & 2DKP             & Indoor                      & 88484                    & 11 & 12       & -       & O                            & 84.69                                       & 112.31                            \\
COCO-Wholebody \citep{Jin2020} & 2DKP             & Outdoor & 40055         & 40055 & -    & -       & -                                      & 85.27                          & 95.51                             \\
Instavariety \citep{Kanazawa2019}            & 2DKP             & Outdoor                         & 2187158       & >28272 & -   & -  & -                    & 88.93                                      & 98.74                             \\
COCO \citep{Lin2014}                         & 2DKP             & Outdoor                         & 28344         & 28344 & -   & -    & -                          & 93.18                   & 97.72                             \\
MuPoTs-3D \citep{Mehta2018} *  & 2DKP             & Outdoor                         & 20760             & 8 & -  & 12      &                            & 95.83                                      & 137.60                             \\
LIP \citep{Gong2017}                      & 2DKP             & Outdoor                         & 25553              & 25553   & -   & -   & -                          & 96.47                            & 113.09                            \\
MPII \citep{Andriluka2014}                     & 2DKP             & Outdoor                         & 14810         & 14810 & 3913  & -  & -                            & 98.18                                 & 121.46                            \\
Crowdpose \citep{Li2019}               & 2DKP             & Outdoor                         & 13927            & -  &-  & -      & P                   & 99.97                                      & 123.47                            \\
Vlog People \citep{Kanazawa2019}                     & 2DKP             & Outdoor                         & 353306        & 798 &798   & -    & -                               & 100.38                                 & 121.42                            \\
PoseTrack (PT) \citep{Andriluka2018}                & 2DKP             & Outdoor                         & 5084          &550 &550    & -    & -                             & 105.30                                  & 135.05                            \\
LSP \citep{Johnson2010}                      & 2DKP             & Outdoor                         & 999           & 999 & -    & -       & -                                & 111.45                            & 153.36                            \\
AI Challenger \citep{Wu2017}                      & 2DKP             & Outdoor                         & 378374        & - & -    & - & -                                & 111.66                         & 115.07                            \\
LSPET \citep{Johnson2011}                     & 2DKP             & Outdoor                         & 9427       & 9427 & -    & -      & -                           & 112.26                        & 125.44                            \\
Penn-Action \citep{Zhang2013}            & 2DKP             & Outdoor                         & 17443       & 2326      & 2326   & -    & -                        & 114.53                                 & 130.17                            \\
OCHuman (OCH) \citep{Zhang2019}                  & 2DKP             & Outdoor                         & 10375    & 8110 & -   & -      & P,O                                   & 130.55                                     & 131.77                            \\
MuCo-3DHP (MuCo) \citep{Mehta2018}               & 2DKP/ 3DKP       & Indoor                         & 482725         & 8 & -   & 14       & P                        & 78.05                                   & 106.08                            \\
MPI-INF-3DHP (MI) \citep{Mehta2017}           & 2DKP/ 3DKP       & Indoor                         & 105274       & 8 & 1     & 14   & -                              & 107.15                         & 132.49                            \\
3DOH50K (OH) \citep{Zhang2020}                 & 2DKP/ 3DKP       & Indoor                         & 50310        & -  & 1   & 6      & O                        & 114.48                                   & 132.38                            \\
3D People \citep{Pumarola2019}                & 2DKP/ 3DKP       & Indoor                         & 1984640       & 80  & -   & 4 & -                               & 108.27                            & 125.44                            \\
AGORA \citep{Patel2021}                    & 2DKP/ 3DKP/ SMPL & Indoor                         & 100015         & >350  & -  & -       & P,O                                & 77.94                 & 105.22                            \\
SURREAL \citep{Varol2017}                  & 2DKP/ 3DKP/ SMPL & Indoor                         & 1605030       & 145  & 2607    & -    & -                              & 110.00                       & 149.99                            \\
Human3.6M (H36M) \citep{Ionescu2014}                     & 2DKP/ 3DKP/ SMPL & Indoor                         & 312188       & 9  & 1     & 4    & -                          & 124.55                                   & 52.68                             \\
EFT-COCO \citep{Joo2021}                & 2DKP/ SMPL       & Outdoor                         & 74834         & 74834 & -    & -     & -                             & 60.82                               & 72.87                             \\
EFT-COCO-part \citep{Joo2021}           & 2DKP/ SMPL       & Outdoor                         & 28062       & 28062 & -    & -               & -               & 67.81                                     & 82.36                             \\
EFT-PoseTrack \citep{Joo2021}            & 2DKP/ SMPL       & Outdoor                         & 28457       & 550 & -     & -     & -                         & 75.17                                    & 94.74                             \\
EFT-MPII \citep{Joo2021}                 & 2DKP/ SMPL       & Outdoor                         & 14667     & 3913 & -     & -     & -                               & 77.67                          & 93.77                             \\
UP-3D \citep{Lassner2017}                    & 2DKP/ SMPL       & Outdoor                         & 7126        & 7126 & -   & -    & -                                & 86.92                              & 181.7                                \\
MTP \citep{Muller2021}                     & 2DKP/ SMPL       & Outdoor                         & 3187           & 3187 & -    & -      & -                            & 87.03                                & 93.69                             \\
EFT-OCHUMAN \citep{Joo2021}              & 2DKP/ SMPL       & Outdoor                         & 2495        & 2495 & -   & -       & P,O                              & 93.44                            & 109.85                            \\
EFT-LSPET \citep{Joo2021}                & 2DKP/ SMPL       & Outdoor                         & 2946       & 2946 & -     & -               & -                & 100.53                                 & 112.03                            \\
3DPW \citep{VonMarcard2018}                    & SMPL             & Outdoor                         & 22735    & 7 & -   & -   & -                                & 89.36                     & 130.63                            \\ \Xhline{1pt}
\end{tabular}
\end{table}
